Overcoming Mode Collapse with Adaptive Multi Adversarial Training

Generative Adversarial Networks (GANs) are a class of generative models used for various applications, but they have been known to suffer from the mode collapse problem, in which some modes of the target distribution are ignored by the generator. Investigative study using a new data generation procedure indicates that the mode collapse of the generator is driven by the discriminator's inability to maintain classification accuracy on previously seen samples, a phenomenon called Catastrophic Forgetting in continual learning. Motivated by this observation, we introduce a novel training procedure that adaptively spawns additional discriminators to remember previous modes of generation. On several datasets, we show that our training scheme can be plugged-in to existing GAN frameworks to mitigate mode collapse and improve standard metrics for GAN evaluation.

==> algos.tex <==
% \begin{algorithm}[H]
% \DontPrintSemicolon
% \SetAlgoLined
% \SetNoFillComment
% % \LinesNotNumbered 
% \SetAlgoLined
% \textbf{Input: }{ Mean $\{\mu_i\}_{i=1}^K$ and standard deviation $\{\sigma_i\}_{i=1}^K$  for initialization,  $\{g_i\}_{i=1}^{L}$ well conditioned $\mathbb{R}^2 \rightarrow \mathbb{R}^2$ functions }\; 
% {
%   Sample weights $\vw \sim \text{Dirichlet}(K)$\;
% $ \mathbf{x}_{2D} \sim \Sigma_{i = 1}^N w_i \mathcal{N}( \mu_i, \sigma_i)$ \tcc*{sample from 2D mixture of gaussians}
% $\mathbf{x}^0_{2D} = \Big[[x^0_{2D}; \mathbbm{1}], [x^1_{2D}; \mathbbm{1}] \Big] $\;
% \tcc{Randomly Init Normalizing Flow}
% \For{$k = 1$ to $k = K$}{  
%     % \If{ $\max(\mM[k]) > \alpha_t * \E_{\ve}(\mM[i])$}{
%     %     Initialize $D_{K+1}$ and optimizer_{K+1}\\
%     %     $\{D_k\} \leftarrow D_{K+1}$\;
%     %     $K \leftarrow K+1$\\
%     %     \textbf{return} $\{D_k\}$
%     % }
%     \textbf{if} k is even \textbf{do} $\vx^k = \big[\vx^{k}_0, \vx^{k}_1 \cdot  g_1(\vx^k_0)\big] $  \;
%     \textbf{if} k is odd \textbf{do}
%     $\vx^k = \big[\vx^{k}_0, \vx^{k}_1 \cdot  g_1(\vx^k_0)\big] $  \
% }
% }
% \caption{Synthetic Data Generation}
% \label{algo:synthetic}
% \end{algorithm}



% \begin{algorithm}[H]
% \DontPrintSemicolon
% \SetAlgoLined
% \SetNoFillComment
% % \LinesNotNumbered 
% \SetAlgoLined
% \textbf{Require:}{ Exemplar Data $\{\ve\}_{i=1}^m$ }\;
% \textbf{Input:}{ Current Discriminator set $\displaystyle \sD = \{f_w^{i}\}_{i=1}^K$}\;
% \For{$i = 1$ to $i = m$}{
% $\vs[k] \leftarrow f_w^{k}(\ve_i) \ \forall\  k\  \in \{1 \dots K\}$\;
%     \If{ $K *\max(\vs) > \alpha_t * \sum_k\vs[k]$}{
%          Initialize $f_w^{K+1}$ with random weights $w$\\
%          $\displaystyle \sD \leftarrow \{f_w^{i}\}_{i=1}^K \bigcup f_w^{K+1}$\tcp*{Append the new discriminator} 
%          \textbf{break}
%         % $K \leftarrow K+1$\\
%         % $T_t \leftarrow T_{t+1}$ \\
%         % % \textbf{return} $\{D_k\}$
        
%     }
% }
% \textbf{return} Discriminator set $\displaystyle \sD$
% \caption{DSPAWN: Discriminator Spawning Subroutine}
% \label{algo:spawn}
% \end{algorithm}
% \begin{figure}
\begin{minipage}[b]{.46\textwidth}
\begin{algorithm}[H]
\DontPrintSemicolon
% \SetAlgoLined
\SetNoFillComment
% \LinesNotNumbered 
% \SetAlgoLined
\begin{algorithmic}
\STATE \textbf{Input:} Mean $\{\mu_i\}_{i=1}^K$ and standard deviation $\{\sigma_i\}_{i=1}^K$  for initialization,  $\{g_i\}_{i=1}^{L}$ well conditioned $\mathbb{R}^2 \rightarrow \mathbb{R}^2$ functions  
\STATE Sample weights $\vw \sim \text{Dirichlet}(K)$ \newline \tcc*{Sample from 2D gaussian mixture}
\STATE $\mathbf{x}_{2D} \sim \Sigma_{i = 1}^N w_i \mathcal{N}( \mu_i, \sigma_i)$  
\STATE $\mathbf{x}^0_{2D} = \Big[[x^0_{2D}; \mathbbm{1}], [x^1_{2D}; \mathbbm{1}] \Big] $ \newline
\tcc*{Randomly Init Normalizing Flow}
\FOR{$k = 1$ to $k = K$}
    % \newline \tcc*{Alternate Identity mapping} \newline
    \IF{k is even} 
    $\vx^k = \big[\vx^{k}_0, \vx^{k}_1 \cdot  g_k(\vx^k_0)\big] $  
    \ELSE
    % \IF{k is odd} 
    $\vx^k = \big[\vx^{k}_0 \cdot  g_k(\vx^k_1), \vx^{k}_1 \big] $  
    \ENDIF
\ENDFOR
\end{algorithmic}
\caption{Synthetic Data Generation}
\label{algo:synthetic}
\end{algorithm}
\vspace{-4mm}
% \end{minipage}
\begin{algorithm}[H]
\DontPrintSemicolon
% \SetAlgoLined
\SetNoFillComment
% \LinesNotNumbered 
% \SetAlgoLined
\caption{DSPAWN: Discriminator \mbox{Spawning} Routine}
\label{algo:spawn}
\begin{algorithmic}
\STATE \textbf{Require:} Exemplar Data $\{\ve\}_{i=1}^m$ 
\STATE \textbf{Input:} Discriminator set $\displaystyle \sD = \{f_w^{i}\}_{i=1}^K$ \newline \tcc*{Check forgetting on exemplars}
\FOR{$i = 1$ to $i = m$}
\STATE $\vs[k] \leftarrow f_w^{k}(\ve_i) \ \forall\  k\  \in \{1 \dots K\}$\;
    \IF{ $K *\max(\vs) > \alpha_t * \sum_k\vs[k]$}
         \STATE Initialize $f_w^{K+1}$ with random weights $w$ \newline \tcc*{Spawn a new discriminator} 
         \STATE Initialize random weight $w^{K+1}$
         \STATE $\displaystyle \sD \leftarrow \{f_w^{i}\}_{i=1}^K \bigcup f_w^{K+1}$
         \STATE \textbf{break}
    \ENDIF
\ENDFOR
\STATE \textbf{return} Discriminator Set $\displaystyle \sD$
\end{algorithmic}
\end{algorithm}
\end{minipage}\hfill
% \end{minipage}\hfill% This must go next to `\end{minipage}`
\begin{minipage}[b]{.48\textwidth}
\begin{algorithm}[H]
\caption{A-MAT: Adaptive Multi-Adversarial Training}
\label{algo:multi}
\DontPrintSemicolon
% \SetAlgoLined
% \SetNoFillComment
% \LinesNotNumbered 
\begin{algorithmic}
\STATE \textbf{Require: }$\vw^{i}_0$, $\vtheta_0$  initial discriminator \& generator params, greediness param $\epsilon$, $\{T_k\}$ spawn warmup iteration schedule

\STATE $\displaystyle \sD \leftarrow \{f_w^{0}\}$\;
\WHILE{$\vtheta$ has not converged}
  \STATE Sample $\{\vz^{(i)}\}_{i=1}^B \sim p(z)$
  \STATE Sample $\{\vx^{(i)}\}_{i=1}^B \sim \mathbb{P}_r$ 
  \STATE Sample $\{\sigma_1(i)\}_{i=1}^B \sim \text{Uniform}(1, K)$
  \STATE Sample $\{\alpha(i)\}_{i=1}^B \sim \text{Bernoulli}(\epsilon)$ \newline \tcc*{Loss weights over discriminators}
  \STATE Sample weights $\vm \sim \text{Dirichlet}(K)$ 
  \STATE $\hat\vx^{(i)} \leftarrow g_\theta(\vz^{(i)}) $  
  \STATE $\sigma_2(i) \leftarrow \argmin_{k}f_w^{k}(\hat\vx^{(i)})$ \newline \tcc*{Discriminator responsible for $\hat{x}^{(i)}$}
  \STATE $\sigma_{z}(i) \leftarrow \alpha(i) \sigma_1(i) + (1 - \alpha(i)) \sigma_2(i)$ \newline \tcc*{Discriminator responsible for $x^{(i)}$} 
  \STATE $\sigma_x(i) \leftarrow \sigma_1(i)$ \newline \tcc*{Training Discriminators}
    $L_{w} \leftarrow \sum_{i=1}^B [f_w^{\sigma_{x}(i)}(\vx_i) - 1]^{-} -  [f_w^{\sigma_{z}(i)}(\hat\vx_i) + 1]^+$
  \FOR{$k = 1$ to $k = \vert \displaystyle \sD \vert$}
     $w^k \leftarrow \text{ADAM}(L_{w})$
  \ENDFOR \newline \tcc*{Training Generator}
  \STATE $s[k] \leftarrow \sum_{i=1}^B f_w^{k}(\hat\vx^{(i)}) \ \forall\  k\  \in \{1 \dots \vert \displaystyle \sD \vert\}$\newline
%   sorted\_indices $\leftarrow$ argsort(D\_score)\;
 \tcc*{Weighed mean over discriminators}
  \STATE $L_{\theta} \leftarrow \text{sort}(\vm) \cdot \text{sort}(s) $
  \STATE $\theta \leftarrow \text{ADAM}(L_{\theta})$\;
%   loss $\leftarrow  -\E_{\vz}[ \sum_{K}\text{weights}[k]*D_{\text{sorted\_indices}[k]}(G(\vz)) ]
    % \tcp*{Check condition to add $D_{K+1}$}
    \IF{more than $T_t$ warm-up iterations since the last spawn}
        $\displaystyle \sD \leftarrow \text{DSPAWN}(\{f_w^{i}\})$
    \ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}
\vspace{-3mm}
\end{minipage}
% \end{figure}

% \raggedbottom


==> tab_synthetic.tex <==
\begin{table*}[t]
\vspace{1mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c||c}
% \hline
\begin{tabular}{c}
$g(\mathbf{z}) = $ 
\end{tabular} 
& $\mathbbm{1}$ 
& \begin{tabular}[c]{@{}c@{}} 
$\mathbf{A}_{392 \times 2}$ 
\\ \end{tabular} & 
\begin{tabular}[c]{@{}c@{}}
$\mathbf{z}$
\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}
MLP 
\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}
MLP, $\mathbf{A}_{392 \times 2}$ 
\end{tabular} 
& \begin{tabular}{@{}c@{}}
\small{MNIST} \end{tabular} 
\\[1ex]
\hline
\begin{tabular}[c]{@{}c@{}}
Label\\ \end{tabular} 
& {\fontfamily{lmtt}\selectfont Level I}      
& {\fontfamily{lmtt}\selectfont Level II}
& {\fontfamily{lmtt}\selectfont Level III}
& {\fontfamily{lmtt}\selectfont Level IV}
& {\fontfamily{lmtt}\selectfont Level V}
& -
\\ 
\hline
\begin{tabular}[c]{@{}c@{}}
\small{GAN-NS \citep{goodfellow2014generative}}\\ \end{tabular} 
& \cmark \enskip \big\vert \enskip  \xmark     
& \cmark \enskip \big\vert \enskip \xmark 
& \cmark \enskip \big\vert \enskip \cmark 
& \cmark \enskip \big\vert \enskip  \cmark 
& \cmark \quad   \big\vert \quad   \cmark
& \xmark 
\\ 
\begin{tabular}[c]{@{}c@{}}
\small{WGAN} \citep{arjovsky2017wasserstein} \\ \end{tabular}    
& \xmark \enskip \big\vert \enskip \xmark      
& \cmark \enskip \big\vert \enskip \xmark
& \cmark \enskip \big\vert \enskip \xmark
& \cmark \enskip \big\vert \enskip   \cmark  
& \cmark \quad   \big\vert \quad   \cmark 
& \xmark 
\\ 
\begin{tabular}[c]{@{}c@{}}
\small{Unrolled GAN} \citep{metz2016unrolled} \end{tabular}
&  \xmark \enskip \big\vert \enskip \xmark
&  \xmark \enskip \big\vert \enskip \xmark 
&  \xmark \enskip \big\vert \enskip \xmark 
&  \xmark \enskip \big\vert \enskip \xmark 
&  \cmark \quad   \big\vert \quad   \cmark    
&  \xmark 
\\
% \end{tabular}

\begin{tabular}[c]{@{}c@{}}
\small{D2GAN} \citep{nguyen2017dual} \end{tabular}
&  \xmark \enskip \big\vert \enskip \xmark
&  \xmark \enskip \big\vert \enskip \xmark
&  \xmark \enskip \big\vert \enskip \xmark
&  \xmark \enskip \big\vert \enskip \xmark
&  \cmark \quad   \big\vert \quad   \cmark
&  \xmark 
\\
% \end{tabular}

\begin{tabular}[c]{@{}c@{}}
\small{GAN-NS + DMAT}  \end{tabular}
&  \xmark \enskip \big\vert \enskip \xmark
&  \xmark \enskip \big\vert \enskip \xmark
&  \xmark \enskip \big\vert \enskip \xmark
&  \xmark \enskip \big\vert \enskip \xmark
&  \cmark \quad   \big\vert \quad   \cmark
&  \xmark 
\\
\end{tabular}
\vspace{3mm}
\caption{\xmark \hspace{0.1mm} indicates that the generator could effectively learn all the data modes, while \cmark \hspace{0.1mm} means \textit{despite best efforts with tuning} the training suffers from mode collapse (more than a quarter of data modes dropped). We show results with the SGD (left) \& ADAM (right) optimizers. MNIST results with ADAM optimizer are provided for reference. We observe that MNIST is a relatively easy dataset, falling between {\fontfamily{lmtt}\selectfont Level I} and {\fontfamily{lmtt}\selectfont II} in terms of complexity.}
\label{tab:synthetic}
}
\end{table*}

